SPBERT: An Efficient Pre-training BERT on SPARQL Queries for Question Answering over Knowledge Graphs

In this paper, we propose SPBERT, a transformer-based language model pre-trained on massive SPARQL query logs. By incorporating masked language modeling objectives and the word structural objective, SPBERT can learn general-purpose representations in both natural language and SPARQL query language. We investigate how SPBERT and encoder-decoder architecture can be adapted for Knowledge-based QA corpora. We conduct exhaustive experiments on two additional tasks, including SPARQL Query Construction and Answer Verbalization Generation. The experimental results show that SPBERT can obtain promising results, achieving state-of-the-art BLEU scores on several of these tasks.

==> checklist.tex <==
For all papers, please check if you include:
- Clear statement of the claims, and how the results substantiate the claims. 
- Description of  any limitations and technical assumptions.
- Conceptual outline and/or pseudocode of methods and algorithms introduced.
- Analysis of the complexity (time, space, sample size) of any algorithm.

For papers including theoretical contributions, please check if you include:
- Formal statement of novel claims (e.g., in theorem statements). 
- Proofs/proof sketches of all novel claims. 
- Citations to theoretical tools used. 

For papers relying on or contributing data sets or ontologies, please check if you include:
- Links to all novel datasets or ontologies introduced (or data/ontologies are included in a data appendix). 
- Links and/or citations of all datasets or ontologies from existing literature.
- Relevant description and statistics of all datasets or ontologies (even those not publicly available). 

For papers including computational experiments, please check if you include: 
- All source code required for conducting the experiments (through a link or a code appendix).
- Descriptions of any external dependencies, including versions, of the source code.
- Specification of the computing infrastructure used for running experiments (hardware and software).
- Evaluation metrics used and the motivation for choosing these metrics.
- All final parameters used in experiments, the range of values tried, and the criterion for selecting the final parameter setting. 
- Result analysis beyond single-dimensional summaries of performance (e.g., average; median), such as measures of variation, confidence, or other distributional information.


==> table/accuracy_score.tex <==
\def\arraystretch{1.2}% 
\setlength{\tabcolsep}{0.9em} %

\begin{table}[htbp]
\centering
\caption{EM metric experiment results on SPARQL Query Construction}
\begin{tabular}{p{3.2cm}|P{1cm}|P{1cm}|P{1cm}|P{1cm}|P{1cm}}
\hline
\centering\textbf{Model} & \textbf{QALD} & \textbf{Mon} & \textbf{Mon50} & \textbf{Mon80} & \textbf{LC-QuAD}  \\

\hline

RNN-Luong & 5.33 & 76 & 85.38 & 89.93 & 1.20 \\
Transformer & 6.00 & 91 & 84.70 & 85.80 & 7.80 \\
ConvS2S & 5.33 & 95 & 90.91 & 90.87 & 8.20 \\
\hline
\hline
BERT2RND & \textbf{6.67} & 96 & 90.69 & 91.35 & 14.80 \\
BERT2BERT &  \textbf{6.67} & 96 & 90.99 & 91.55 & 18.00 \\
\hline
\hline

\textbf{MLM} &&&&& \\
- BERT2SPBERT (S) &  \textbf{6.67} & \textbf{97} & 90.80 & 92.22 & 12.40 \\
- BERT2SPBERT (B) &  \textbf{6.67} & 95 & \textbf{91.18} & \textbf{92.70} & \textbf{20.20} \\

\textbf{MLM + WSO} &&&&&\\
- BERT2SPBERT (B) &  \textbf{6.67} & 96 & 90.84 & 91.75 & 16.80 \\

\hline
\end{tabular}
\label{em_table}
\end{table}

==> table/bleu_score.tex <==
\def\arraystretch{1.2}% 
\setlength{\tabcolsep}{0.9em} %

\begin{table}[htbp]
\centering
\caption{BLEU score experiment results on SPARQL Query Construction}
\begin{tabular}{p{3.2cm}|P{1cm}|P{1cm}|P{1cm}|P{1cm}|P{1cm}}
\hline
\centering \textbf{Model} & \textbf{QALD} & \textbf{Mon} & \textbf{Mon50} & \textbf{Mon80} & \textbf{LC-QuAD}  \\

\hline

RNN-Luong & 31.77 & 91.67 & 94.75 & 96.12 & 51.06 \\
Transformer & 33.77 & 95.31 & 93.92 & 94.87 & 57.43 \\
ConvS2S & 31.81 & 97.12 & \textbf{96.62} & 96.47 & 59.54 \\
\hline
\hline
BERT2RND & 34.36 & 97.03 & 95.28 & 96.44 & 66.52 \\
BERT2BERT & 35.86 & 97.03 & 96.20 & 96.14 & \textbf{68.80} \\
\hline
\hline

\textbf{MLM} &&&&& \\
- BERT2SPBERT (S) & 35.19 & 97.28 & 96.06 & 96.29 & 64.18 \\
- BERT2SPBERT (B) & 35.95 & 96.78 & 96.45 & \textbf{96.87} & 68.08 \\

\textbf{MLM + WSO} &&&&&\\
- BERT2SPERT (B) &  \textbf{37.58} & \textbf{97.33} & 96.20 & 96.36 & 68.35 \\

\hline
\end{tabular}
\label{bleu_table}
\textit{Notes:}  We train SPBERT (third group) from scratch (S) or initialized with the parameters of BERT (B), and we also use different learning objectives (only MLM, the combination of MLM and WSO). The best scores are in bold.
\end{table}

==> table/lowresource_table.tex <==
\def\arraystretch{1.2}% 
\setlength{\tabcolsep}{0.9em} %

\begin{table}[htbp]
\centering
\caption{BLEU score experiment results on QALD-9 Dataset}
\begin{tabular}{p{3.2cm}|P{1cm}|P{1cm}|P{1cm}}
\hline
\centering\textbf{Model} & \textbf{En} & \textbf{De} & \textbf{Fr} \\

\hline

RNN-Luong & 22.29 & 21.33 & 34.34 \\
Transformer & 24.16 & 22.98 & 31.65\\
ConvS2S & 26.02 & 25.95 & 32.61 \\
\hline
\hline
BERT2RND & 100.00 & 100.00 & 100.00 \\
BERT2BERT & 100.00 & 100.00 & 100.00  \\
\hline
\hline

\textbf{MLM} &&& \\
- BERT2SPBERT (S) & 100.00 & 100.00 & 100.00  \\
- BERT2SPBERT (B) & 100.00 & 100.00 & 100.00 \\

\textbf{MLM + WSO} &&&\\
- BERT2SPBERT (B) & 100.00 & 100.00 & 100.00 \\

\hline

\end{tabular}
\label{qald_table}

\end{table}
